An Empirical Study of Accuracy-Robustness Tradeoff and Training Efficiency in Self-Supervised Learning

Self-supervised learning (SSL) has significantly advanced image representation learning, yet efficiency challenges persist, particularly with adversarial training. Many SSL methods require extensive epochs to achieve convergence, a demand further amplified in adversarial settings. To address this inefficiency, we revisit the robust EMP-SSL framework, emphasizing the importance of increasing the number of crops per image to accelerate learning. Unlike traditional contrastive learning, robust EMP-SSL leverages multi-crop sampling, integrates an invariance term and regularization, and reduces training epochs, enhancing time efficiency. Evaluated with both standard linear classifiers and multi-patch embedding aggregation, robust EMP-SSL provides new insights into SSL evaluation strategies. Our results show that robust crop-based EMP-SSL not only accelerates convergence but also achieves a superior balance between clean accuracy and adversarial robustness, outperforming multi-crop embedding aggregation. Additionally, we extend this approach with free adversarial training in Multi-Crop SSL, introducing the Cost-Free Adversarial Multi-Crop Self-Supervised Learning (CF-AMC-SSL) method. CF-AMC-SSL demonstrates the effectiveness of free adversarial training in reducing training time while simultaneously improving clean accuracy and adversarial robustness. These findings underscore the potential of CF-AMC-SSL for practical SSL applications. Our code is publicly available at https://github.com/softsys4ai/CF-AMC-SSL.

==> comments.tex <==
In this section, we explain the methodology of our comparative study on the robustness of two learning schemes including baseline self-supervised contrastive learning (SimCLR) \cite{chen2020simple} and Extreme-Multi-Patch Self-Supervised-Learning (EMP-SSL) \cite{tong2023emp} algorithms.

Initially, our analysis in Table \ref{table: ST-simclr-vs-EMP} reveals that both the baseline EMP-SSL and SimCLR are vulnerable to adversarial attacks. This finding further underscores the lack of robustness in SimCLR, consistent with previous research findings \cite{ghofrani2023rethinking, kim2020adversarial}. To enhance their robustness, we employ adversarial training, as depicted in Figure \ref{EMP}.


\subsection{Robust SimCLR: A Simple Framework for Contrastive Learning with Adversarial Training}

SimCLR uses data augmentation to create positive pairs of augmented images from each original image. The contrastive loss function encourages the model to learn similar representations for these positive pairs while distinguishing them from other negative samples. To enhance robustness through adversarial training (see Fig. \ref{fig:contrastive}):

\begin{enumerate}
    \item Adversarial examples are generated for each image in a mini-batch. For each original image, both its augmented version and the adversarial counterpart are treated as positive pairs.
    \item The contrastive loss function is updated to incorporate these adversarial pairs, aiming to maintain similarity between adversarial and original augmented views while distinguishing them from other negative samples.
    % \item The updated contrastive loss with adversarial training is:
    % \[
    % \mathscr{L}_{\text{adv}} = \frac{1}{2\,|S|} \sum \left(l_{i,j}^{\text{adv}} + l_{j,i}^{\text{adv}}\right)
    % \]
    % where \( |S| \) denotes the number of positive pairs in the dataset, and:
    % \[
    % l_{i,j}^{\text{adv}} = -\log\left(\frac{\exp\left(\frac{sim(\bm{z}_i, \bm{z}_j^{\text{adv}})}{\tau}\right)}{\sum_{k \neq i} \exp\left(\frac{sim(\bm{z}_i, \bm{z}_k)}{\tau}\right)}\right)
    % \]
    % Here, $\bm{z}_j^{\text{adv}}$ denotes the adversarial perturbation of $\bm{z}_j$.
\end{enumerate}
\subsection{Robust EMP-SSL: Extreme-Multi-Patch Self-Supervised Learning with Adversarial Training}

EMP-SSL applies multiple fixed-scale patches per image. We incorporate adversarial training into EMP-SSL as follows (see Fig. \ref{fig:EMP-SSL}):

\begin{enumerate}
    \item $C$ adversarial examples from $C$ augmented versions of each image are generated.
    \item The training objective is updated to include these adversarial examples. The revised training objective is:
    \[
    \max \frac{1}{n}\sum_{i=1, \ldots, n} \left( R(Z_i^{\text{adv}}) + \lambda D(Z_i^{\text{adv}}, \bar{Z}_{\text{adv}}) \right)
    \]
    where:
    \[
    R(Z_i^{\text{adv}}) = \frac{1}{2} \log \det \left( I + \frac{d}{b\epsilon^2} Z_i^{\text{adv}} (Z_i^{\text{adv}})^T \right)
    \]
    and:
    \[
    D(Z_i^{\text{adv}}, \bar{Z}_{\text{adv}}) = \text{Tr}\left((Z_i^{\text{adv}})^T \bar{Z}_{\text{adv}}\right)
    \]
    Here, \( \bar{Z}_{\text{adv}} \) is the average representation of adversarial examples, and \(\lambda\) is a weight parameter for invariance loss.
\end{enumerate}


\subsection{Theoretical Analysis}

The CF-AMC-SSL method, with its regularization and invariance terms, achieves a better balance between clean accuracy and adversarial robustness compared to SimCLR with adversarial training. We can provide a mathematical justification for this balance as follows:

\subsubsection{Regularization Term: \( R(Z_i^{\text{adv}}) \)}

In CF-AMC-SSL, the regularization term is expressed as:

\[
R(Z_i^{\text{adv}}) = \frac{1}{2} \log \det \left( I + \frac{d}{b\epsilon^2} Z_i^{\text{adv}} (Z_i^{\text{adv}})^T \right)
\]

This term penalizes high correlations between the dimensions of the adversarial representation \( Z_i^{\text{adv}} \). Here's how:

\begin{itemize}
    \item \textbf{Covariance and Correlation:} The matrix \( Z_i^{\text{adv}} (Z_i^{\text{adv}})^T \) represents the covariance matrix of the adversarial features. The determinant of this matrix, \( \det(Z_i^{\text{adv}} (Z_i^{\text{adv}})^T) \), is related to the product of the eigenvalues of the covariance matrix.
    \item \textbf{Penalizing Overfitting to Style:} A high determinant suggests that the eigenvalues are large, implying that the model may be capturing style-specific features rather than content. The logarithm of the determinant in \( R(Z_i^{\text{adv}}) \) penalizes these large eigenvalues, thereby reducing the model's tendency to overfit to style-induced perturbations.
    \item \textbf{Content Focus:} By penalizing large eigenvalues, the regularization term forces the model to focus on features that are consistent (i.e., content-based) rather than those that vary with different styles. This ensures that the adversarial representations remain tied to the content \( c \), which is invariant across different styles.
\end{itemize}

In SimCLR with adversarial training, there is no explicit regularization term that penalizes correlations in the adversarial representations. This can lead to overfitting to adversarial examples, where the model may prioritize robustness over content preservation, potentially degrading clean accuracy.

\subsubsection{Invariance Term: \( D(Z_i^{\text{adv}}, \bar{Z}_{\text{adv}}) \)}

The invariance term in CF-AMC-SSL is expressed as:

\[
D(Z_i^{\text{adv}}, \bar{Z}_{\text{adv}}) = \text{Tr}\left((Z_i^{\text{adv}})^T \bar{Z}_{\text{adv}}\right)
\]

This term enforces consistency between the adversarial representation \( Z_i^{\text{adv}} \) and the average adversarial representation \( \bar{Z}_{\text{adv}} \):

\begin{itemize}
    \item \textbf{Trace and Alignment:} The trace operation \( \text{Tr}\left((Z_i^{\text{adv}})^T \bar{Z}_{\text{adv}}\right) \) sums the diagonal elements of the matrix product \( (Z_i^{\text{adv}})^T \bar{Z}_{\text{adv}} \), which is a measure of alignment between the individual adversarial representation \( Z_i^{\text{adv}} \) and the average representation \( \bar{Z}_{\text{adv}} \).
    \item \textbf{Smoothness:} By maximizing this alignment, the invariance term ensures that the representations of adversarial examples are not only robust but also consistent across different augmentations and perturbations. This consistency leads to smoother representations that are less sensitive to specific adversarial perturbations, thereby preserving clean accuracy.
\end{itemize}

In SimCLR with adversarial training, which typically uses only two augmentations, the lack of a robust invariance mechanism can lead to variability in the representations of adversarial examples. This variability might cause the model to overfit to adversarial noise, leading to a trade-off where adversarial robustness is gained at the expense of clean accuracy.

\subsubsection{Combined Effect on Balance between Clean Accuracy and Adversarial Robustness}

The CF-AMC-SSL method's dual mechanisms (regularization and invariance terms) provide a mathematically grounded approach to balancing clean accuracy and adversarial robustness:

\[
\text{Objective:} \quad \max \frac{1}{n}\sum_{i=1}^{n} \left( R(Z_i^{\text{adv}}) + \lambda D(Z_i^{\text{adv}}, \bar{Z}_{\text{adv}}) \right)
\]

\begin{itemize}
    \item \textbf{Regularization Term:} Ensures that the representations are content-focused, reducing overfitting to adversarial perturbations and thereby preserving clean accuracy.
    \item \textbf{Invariance Term:} Promotes consistency and smoothness across adversarial examples, ensuring robustness without sacrificing generalization to clean data.
\end{itemize}

In contrast, SimCLR with adversarial training lacks these explicit mechanisms, which may lead to a suboptimal trade-off where the model becomes overly robust at the expense of clean accuracy. The mathematical structure of CF-AMC-SSL allows it to navigate this trade-off more effectively, leading to better overall performance.

 % Choosing a larger number \( n \) of image patches accelerates learning the co-occurrence between patches, contributing to faster convergence and reduced training time. This choice is a key reason for EMP-SSL’s efficiency compared to SimCLR.
% In this section, we explain the methodology of our comparative study on the robustness of two learning schemes including baseline self-supervised contrastive learning (SimCLR) \cite{chen2020simple} and Extreme-Multi-Patch Self-Supervised-Learning (EMP-SSL) \cite{tong2023emp} algorithms.
% % (see supplementary materials for details) :
% \subsection{Preliminaries}
% Before introducing our approach, we first provide a brief overview of self-supervised contrastive learning with SimCLR and the Extreme-Multi-Patch Self-Supervised Learning (EMP-SSL) algorithms. This will help highlight the key differences between these two frameworks.
% \\

% \textbf{SimCLR: A Simple Framework for Contrastive Learning}
% The SimCLR framework involves applying data augmentation techniques to generate two views of each data point, treating these views as positive pairs during training. SimCLR consists of three main components: the base encoder, responsible for extracting meaningful representations from raw input data; the projection head, which transforms high-dimensional feature vectors into a lower-dimensional space for contrastive loss application; and the contrastive loss function itself. The contrastive loss aims to encourage similar representations for positive pairs while pushing apart representations of dissimilar instances, thereby facilitating improved model performance through effective representation learning.

% % In essence, SimCLR is a self-supervised method that learns meaningful representations by maximizing similarity between similar samples and minimizing it between dissimilar ones.
% % The main idea of this framework is summarized as follows \cite{chen2020simple}:
% % \begin{enumerate}
% %     \item  SimCLR employs strong data augmentation methods to generate diverse views of each data point, treating each view as a positive pair alongside other augmentations of the same data point. Simultaneously, it ensures that the representations of different data points serve as negative samples, encouraging the model to distinguish between dissimilar instances.
% %     \item The base encoder is a neural network responsible for transforming the raw input data (e.g., images, text, audio) into a meaningful representation in a high-dimensional space. It extracts features from the data, which are then used for further learning.
% %     \item The projection head is an additional neural network component applied to the representations generated by the base encoder. Its primary role is to project the high-dimensional feature vectors into a lower-dimensional space where the contrastive loss can be applied. 
% %     \item The contrastive loss function is defined for a set of representations $\lbrace \bm{z}_k \rbrace$, including positive pairs $\bm{z}_i$ and $\bm{z}_j$, as follows:
% %     \begin{equation}
% %     \mathscr{L} = \frac{1}{2\,|S|} \sum \left(l_{i,j} + l_{j,i}\right)
% %     \end{equation}

% % Where the sum is over all positive pairs, and:

% % \begin{equation}
% % l_{i,j} = -\log\left(\frac{\exp\left(\frac{sim(\bm{z}_i,\bm{z}_j)}{\tau}\right)}{\sum_{k\neq i} \exp\left(\frac{sim(\bm{z}_i,\bm{z}_k)}{\tau}\right)}\right)
% % \end{equation}

% % Here, $sim$ represents a similarity measure, and $\tau$ is the temperature parameter of the loss function.
% % \end{enumerate}

% \textbf{EMP-SSL: Extreme Multi Patch Sef-Supervised Learning}
% The main idea of the EMP-SSL algorithm \cite{tong2023emp} is summarized as follows:
% \begin{enumerate}
%   \item Images are first augmented to obtain $n$ sets of augmented images, denoted as $X_1, X_2, \ldots, X_n$, where $X_i = [x_{1i}, x_{2i}, \ldots, x_{bi}]$. Each $X_i$ represents the collection of augmented image patches from a single image in the batch.
  
%   \item These augmented image patches, $X_1, X_2, \ldots, X_n$, are then passed into the encoder to extract features, resulting in feature vectors $Z_1, Z_2, \ldots, Z_n$. These feature vectors are concatenated into $Z = [Z_1, Z_2, \ldots, Z_n]$.

%   \item The training objective is defined as follows, aiming to maximize a combination of Total Coding Rate (TCR) and invariance loss ($\lambda$ is the weight of invariance loss):

%   \[
%   \max \frac{1}{n}\sum_{i=1, \ldots, n} \left( R(Z_i) + \lambda D(Z_i, \bar{Z}) \right)
%   \]

%   where:
  
%   \[
%   R(Z) = \frac{1}{2} \log \det \left( I + \frac{d}{b\epsilon^2} ZZ^T \right)
%   \]
  
%   is the TCR that serves as a covariance regularization technique, aiming to avoid collapsed representations. Here, $b$ is the batch size, $\epsilon$ is the distortion size chosen with $\epsilon > 0$, and $d$ is the dimension of the projection vectors. The distance function is implemented using Cosine Similarity:
  
%   \[
%   D(Z_1, Z_2) = \text{Tr}(Z_1^T Z_2)
%   \]
  
%   A higher value of $D$ indicates a greater similarity between $Z_i$ and $\bar{Z}$.
%   This process combines image augmentation, feature extraction, regularization techniques, and a training objective focused on regularization and invariance to improve the performance of a deep neural network.
% \end{enumerate}
% The main differences between these two frameworks are as follows:
% \begin{itemize}
% \item SimCLR uses two multi-scale crops per image, whereas EMP-SSL utilizes multiple fixed-scale patches per image.
% \item SimCLR requires a significantly higher number of epochs to converge compared to EMP-SSL.
% \item The contrastive loss in SimCLR aims to encourage similar representations for positive pairs (two multi-scale crops per image) while pushing apart representations of dissimilar instances (the rest of the images in the minibatch). Conversely, the loss in EMP-SSL focuses on maximizing the similarity between representations of multiple fixed-scale patches and their averaged representation.
% \end{itemize}
% \subsection{Adversarially Trained SSL}
% Initially, our analysis reveals vulnerabilities in the standard SimCLR and EMP-SSL models in adversarial attacks, as outlined in Table \ref{table: ST-simclr-vs-EMP}. To enhance their robustness, we employ adversarial training, as depicted in Figure \ref{EMP}. In the SimCLR framework, as part of adversarial training, we generate an adversarial example for each image, considering both the augmented version of the original image and the generated adversarial counterpart as positive samples. In contrast, in the EMP framework, we generate $C$ adversarial examples from $C$ augmented versions of an original image. Our objective is to converge these adversarial examples towards their collective average representation, thereby enhancing the model's robustness against adversarial perturbations. 
We implement two distinct strategies to form positive pairs:
\begin{itemize}
\item \textbf{Crop-Based Method}: Involves random selection of image augmentations, ranging in size from 9×9 to 32×32, for sampling.
\item \textbf{Patch-Based Method}: Replaces multi-scale cropping augmentation with a fixed-scale image patch approach.
\end{itemize}
The final algorithm involves adversarially trained EMP-SSL with crop-based augmentations. Note that while using a higher number of patches in joint embedding self-supervised learning may extend the training duration, EMP-SSL demonstrates significant promise. It not only requires fewer training epochs to converge but also exhibits a reduced runtime \cite{tong2023emp}.



% \subsection{Cost-Free Adversarial Multi-Crop Self-Supervised Learning (CF-AMC-SSL)}
% In our proposed method, \textit{Cost-Free Adversarial Multi-Crop Self-Supervised Learning} (\textbf{CF-AMC-SSL}),we begin by adversarially training the SimCLR and EMP-SSL frameworks. We implement two distinct strategies to form positive pairs:
% \begin{itemize}
% \item \textbf{Crop-Based Method}: Involves random selection of image augmentations, ranging in size from 9×9 to 32×32, for sampling.
% \item \textbf{Patch-Based Method}: Replaces multi-scale cropping augmentation with a fixed-scale image patch approach.
% \end{itemize}
% The final algorithm involves adversarially trained EMP-SSL with crop-based augmentations. Although using a higher number of patches in joint-embedding self-supervised learning might extend training duration, EMP-SSL shows promise. It not only requires fewer training epochs to converge but also boasts reduced runtime \cite{tong2023emp}.
\subsection{Towards Adversarial Multi-Crop Self-Supervised Learning in a Few Epochs}

We now describe how to obtain adversarial robustness in the representations within a few epochs (see Figure \ref{EMP}). As stated previously, our initial step involves adversarial training of EMP-SSL. However, to enhance robustness, we transition from patch-based image augmentations to crop-based alternatives. Our findings reveal that using a moderate number of crops enhances model robustness and drastically reduces runtime by almost half compared to the baseline adversarial training in SimCLR. To further speed up the process, we adopt free adversarial training \cite{shafahi2019adversarial}, which simultaneously updates both model parameters and image perturbations using a single backward pass, instead of separate gradient computations for each update step. The training process involves the network processing minibatch forwards and computing parameter gradients backward. With the "free" method, this also computes the loss gradient for the input image simultaneously. However, it limits multiple adversarial updates on the same image without extra backward passes. To overcome this, training on the same minibatch is iterated consecutively for $m$ iterations. Then, the total epochs are divided by $m$ to maintain a consistent total count of training iterations, allowing multiple adversarial updates for each training image.



The **regularization term** indeed plays a role in managing the correlation of features within the learned representations. The goal of this term, particularly in the context of adversarial training, is to ensure that the representations are **robust** and primarily capture the **causal content** rather than overfitting to **style-induced perturbations**. When using **multiple augmentations**, the model is exposed to a broader variety of transformations, which helps in **decorrelating the learned features** from the style information. This broader exposure makes the representations less sensitive to the specific variations in style (e.g., color, texture) that might be introduced by the augmentations or adversarial perturbations. As a result, the features become more **independent of style information** compared to when only two augmentations are used. In essence, with multiple augmentations, the model learns to focus more on the underlying content that remains consistent across different views of the data, thereby improving the generalization and robustness of the learned representations. The regularization term supports this process by discouraging overfitting to any particular style-induced variation, ensuring that the learned features are more **content-focused** and less entangled with the style.
